Finding High-Value Training Data Subset through Differentiable Convex Programming

Finding valuable training data points for deep neural networks has been a core research challenge with many applications. In recent years, various techniques for calculating the "value" of individual training datapoints have been proposed for explaining trained models. However, the value of a training datapoint also depends on other selected training datapoints - a notion that is not explicitly captured by existing methods. In this paper, we study the problem of selecting high-value subsets of training data. The key idea is to design a learnable framework for online subset selection, which can be learned using mini-batches of training data, thus making our method scalable. This results in a parameterized convex subset selection problem that is amenable to a differentiable convex programming paradigm, thus allowing us to learn the parameters of the selection model in end-to-end training. Using this framework, we design an online alternating minimization-based algorithm for jointly learning the parameters of the selection model and ML model. Extensive evaluation on a synthetic dataset, and three standard datasets, show that our algorithm finds consistently higher value subsets of training data, compared to the recent state-of-the-art methods, sometimes ~20% higher value than existing methods. The subsets are also useful in finding mislabelled training data. Our algorithm takes running time comparable to the existing valuation functions.

==> algo.tex <==
\begin{algorithm}
 \caption{: High-Value Subset through Differentiable Convex Programming}
 \label{algo:submodular}
 \begin{algorithmic}[1]
 
 \State \textbf{Input:}
 \State \hspace{2mm} Training dataset $\cD$, Test dataset $\cD^t$
 \State \textbf{Output:}
 \State \hspace{2mm} Model Parameter $\theta$, Embedding model for selection parameter $\phi$
 %\State \hspace{2mm} Test data
%  \State \hspace{2mm} $k$: Subset cardinality
 %\Procedure{Process:}{a}
 \State{\textbf{Algorithm:}}
 \State Training set is partitioned into existing set E and incoming set I which is further partitioned into mini batches $\mathcal{B}$. Let E be initially empty.
 %\hspace{2mm}\For{each minibatch b in $\mathcal{B}$}
 \hspace{2mm}\For{each timestep $t$}
 %\hspace{2mm}\For{each x $\in$ X \textbackslash $S_{i-1}$}
%  \State $Rep_E^{b-1}$ = Pre-trained VGG-16 features($E_{b-1}$)
%  \State $Rep_I^{b}$ = Pre-trained VGG-16 features($I_b$)
\State Extract a minibatch of data $b$ from $\mathcal{B}$
\State We examine pairs of instances from each minibatch. Let $i$ and $j$ be a pair.
\State $u_i$ , $u_j$ = Features (maybe pre-trained) of instance $i$ and $j$
\State Let $D_{ij}^o$ be the pairwise distance between instance i from existing set E and j from incoming set I and $D_{ij}^n$ be the pairwise distance between instance i and j from I. $D_{i,j} = ||(u_i - u_j)||_p$.
%  \State $select_I$ = S($Rep_E^{b-1}, Rep_I^{b}$)
%  \State S($Rep_E^{b-1}, Rep_I^{b}$) 
\State S($D_{ij}^o, D_{ij}^n ; \phi$) is the selection network using representations of existing/representative set E and of incoming mini batch I.
\State Within the selection network parameterized by $\phi$, we solve the convex optimisation problem $argmin_z \sum_{i}\sum_{j} D_{i,j}^o z_{ij}^o + \sum_{ij} D_{i,j}^n z_{ij}^n$ where $z^o$ and $z^n$ are the output variables.
\State $s_j = \frac{1}{\xi} max(\sum_i z_{ij}^n,\xi)$ where $\xi$ is a threshold value. $s_j$ denotes the representative power of instance j from incoming set I.
$s_j$ will be 0 for the unselected instances and 1 for the selected ones.
\State $E \longleftarrow E \bigcup \{j | s_j \geq \xi\}$ : Fill the representative set with selected instances.
\State Initialize an end-task (here, classification) network parameterized by $\theta$.
\State We compute the training loss ($TrLoss$) : $TrLoss(\phi,\theta_{t-1}) = \sum_j s_j(\phi) Loss_j(\theta_{t-1})$ where $j$ is instance indexed from the current mini batch. The gradients will be required to backpropagate through the selected instances only.
\State Compute the joint selection and end-task parameter: $\hat{\theta}_t(\phi,\theta_{t-1})$ = $\theta_{t-1} - \eta \nabla_{\theta} TrLoss(\phi,\theta_{t-1})$
%\State $w_b$ = \textit{Net}($select_I , w_{b-1}$) //Train the network \textit{Net} with the subset.
%  \State  TsLoss = LossN(Test data , $w_b)$
\State Compute the test set loss ($TsLoss$) using $\hat{\theta}_t(\phi,\theta_{t-1})$ :   $TsLoss(\phi,\theta_{t-1}) = \sum_{k\in test data} NewLoss(x_k, y_k , \hat{\theta}_{t}(\phi,\theta_{t-1}))$. This will help in finding the gradients of the test set loss w.r.t the selection parameters $\phi$.
\State We update the selection network parameters: \\ $\phi_t$ = $\phi_{t-1} - \eta \nabla TsLoss(\phi_{t-1})$.
\State We update the end-task network parameters: \\ $\theta_t$ = $\theta_{t-1} - \eta \nabla TrLoss(\phi,\theta_{t-1})$.
 \EndFor
 \State \textbf{Output:}
 \State $E$ : Final representative set
 %\EndProcedure
 \end{algorithmic}
\end{algorithm}

==> method.tex <==
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\psistar}{\Psi^*}
\newcommand{\thetastar}{\Theta^*}
\newcommand{\argmin}{\mbox{arg}\min}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\psihat}{\hat{\Psi}}

%\newtheorem{definition}{Definition}
%\newtheorem{theorem}{Theorem}

In this section, we formally define the problem of valuable subset selection and propose an learned approximate algorithm for the same.

\subsection{Motivation and Problem Formulation}

Data valuation for deep learning is an important tool for generating explanations of deep learning models in terms of training data.
Let $\cD = \{ z_i = (x_i,y_i) | i=1,\dots,n \}$ be the training dataset with $x_i\in \cX$ being the features and $y_i\in \cY$ being the labels. Let $\Psi$ denote the parameters for a machine learning model, which is trained by minimizing a loss function $\cL$ over the training dataset:
 $ \psistar =  \argmin_{\Psi} \cL(\Psi, \cD) = \argmin_{\Psi} \frac{1}{n} \sum_{z_i\in\cD} L(z_i,\Psi)$. 
Also, let $\cV(z_i, \psistar)$ denote the value function using which we evaluate the effectiveness of a training training data point $z_i\in \cD$. Typically, one uses an affine function over a test dataset $\cD^t$ as the value function: 
$$\cV(z_i ;\psistar,\cD^t) = \frac{1}{m} \sum_{z\in\cD^t} V(z; z_i,\psistar) $$
where $m$ is the number of test examples. Note that here the per-test example value function $V(z; z_i,\psistar)$ depends on the optimal model $\psistar$, the training example $z_i$ whose value we are trying to determine, and test example $z$. We shall refer to both $\cV$ and $V$ as \textit{value function}, since the exact connotation is clear from context.

\sbc{redefine the value function as a set function. Let $\cV(S ;\psistar,\cD^t)$ be the value of a subset of training datapoints, $S\subseteq \cD$}

A commonly used value function is the influence function \cite{koh2017understanding}, which computes the value of training example $z_i$ as the rate of change of test loss w.r.t. a weightage $\epsilon$ given to a training datapoint:
\begin{align*}
& \psihat(z_i) = \argmin_{\Psi} [ \cL(\Psi,\cD) + \epsilon L(\Psi, z_i) ] \\
& V(z; z_i,\psistar) = \nabla_{\epsilon} L(z, \psihat) = \nabla_{\psihat} L(z, \psistar) * \nabla_{\epsilon} \psihat(z_i; \psistar)
\end{align*}
%While the above value function does not depend on $\psistar$, 
$\nabla_{\epsilon} \psihat(z_i; \psistar)$ can be calculated for linear models using a result from Cook and Weisberg \cite{cook1982residuals}. $V(z; z_i,\psistar)$ can be positive or negative depending on whether or not the test loss decreases or increases by adding training point. Hence $-V(z; z_i,\psistar)$ captures the ``value'' of training point $z_i$.
Note that here only the effect of removing a single datapoint is captured. The interactions with other datapoints in the training set is not captured.

Another commonly used data valuation technique, which partially addresses this problem is based on Shapley Values \cite{ghorbani2019data}. Shapley value of a given training datapoint $z_i$ is defined as the expected marginal contribution of the training datapoint $z_i$ towards the test loss function, where the expectation is taken of all possible calculated as:
\begin{align*}
\psihat(S,z_i) = \argmin_{\Psi} \cL(\Psi,S\cup\{z_i\}),\  \psihat(S) = \argmin_{\Psi} \cL(\Psi,S) \\
V(z,z_i,\psistar) = \mathbb{E}_{S\sim \mathcal{P}(\cD-\{z_i\})} [L(z,\psihat(S)) - L(z,\psihat(S,z_i)) ]
\end{align*}
Note that $V(z; z_i,\psistar)$ is expected to be positive if $z_i$ decreases the test loss, and vice versa. Note that exact calculation of the expectation takes exponential time in $n$. \cite{ghorbani2019data} provide a monte-carlo algorithm, and a gradient based algorithm for approximating the data Shapley value.

The Data Shapley value function computes the average marginal utility of a given training datapoint $z_i$, over all subsets of other datapoints. This can cause some of the important subsets of training data, which are complementary to $z_i$, to have a lower impact on the valuation of $z_i$. For example, consider a 3-class classification problem where class A shares boundary with two other classes, B and C; and the boundary with class B has a much higher data density than the boundary with class C (see figure \ref{fig:classdv}). Hence, many more subsets of datapoints on boundary with class C will have complementary datapoints than those on the boundary of class B. Hence, the datapoints at the boundary of class C will have much higher Shapley value than those on the boundary of class B. Hence in a ranking for selection of training datapoints, points from boundary of class C will be selected first, followed by points from boundary of class B. Clearly, this is not an ideal ranking. Ideally, high-valued datapoints should include roughly equal number of points from both boundaries, considering that the value function penalizes errors on both sides equally.

\begin{figure}[h!]
    %\centering
    \centering
    \begin{subfigure}{0.6\columnwidth}
    \includegraphics[width=\textwidth,height=4cm]{figures/classes_datavalue.png}
    \end{subfigure}
    \caption{\textbf{Class boundaries of a 3-class classification problem}}
    \label{fig:classdv}
\end{figure}

In this paper, we attempt to correct the above mentioned bias by defining the problem of finding a high-value data subset from the training dataset. Additionally, we bring in the concept of \textit{surrogate model}, which is the function class used to ascertain the value of a training data subset. For example, LIME \cite{ribeiro2016should} uses local linear models as surrogate models for generating explanations. For deep neural networks a natural choice for the surrogate model is a neural network with the same architecture as the original model. However, a different function class may be useful in making the data valuation efficient in a transfer learning context when original neural network is large and only a subset of the layers undergoes changes (e.g. the final layers of image classification after a large Resnet feature encoder). Let $\Theta$ denote the parameters of the surrogate model, and $\thetastar(S)$ be the optimal parameters of the surrogate model when trained on the subset $S\subseteq \cD$ of the training data. We define the \textit{high-value data-subset selection} problem as:

\begin{definition}
\textbf{High-value Data Subset Selection}: Given a training dataset $\cD$ and a value function $\cV(S ;\psistar,\cD^t)$ for a subset $S\subseteq \cD$, let 
$$\thetastar(S) = \argmin_{\Theta} \cL(\Theta,S(\psistar))$$
where $S(\psistar)$ is the subset of training examples, with the label $y$ of the datapoint $(x,y)$ replaced by the predicted label $\psistar(x)$. A high-value data subset $S^*$ is given by:
\[ S^* = \argmin_{S\subseteq \cD} \cV(S, \thetastar(S), \cD^t) \]
\end{definition}

The combinatorial problem of high-value data subset selection as described above is an NP-hard problem, with one of the common solutions is based on a relaxation of the facility location integer programming relaxation of the subset selection problem \cite{abc}. The facility-location formulation has also been extended to online subset selection setting \cite{elhamifar2017online}, which can be used with   has also been extended  In the next section, we describe 

\subsection{Trainable Convex Subset Selection Layer}

\sbc{ Describe the online subset selection formulation, and the layer for it.
Question is why are we not directly taking the selection network as in \cite{yoon2020data} ? }

In this section we describe our formulation of explanation 



\subsection{Online Training of Subset Selection Model}

\sbc{ Describe the formulation where we consider the one step update parameters for surrogate model to be the optimal model and learn the parameters of selection model using the value function on the updated surrogate model.\\
Describe the alternating online optimization algorithm which optimizes the parameter }

% \begin{algorithm}
%  \caption{: Coupled Subset Training}
%  \label{algo:submodular}
%  \begin{algorithmic}[1]
 
%  \State \textbf{Input:}
%  \State \hspace{2mm} Training data
%  \State \hspace{2mm} Test data
% %  \State \hspace{2mm} $k$: Subset cardinality
%  \State \textbf{Process:}\\
%   \hspace{2mm} Training set is partitioned into existing set E and incoming set I which is further partitioned into mini batches $\mathcal{B}$. Let E be initially empty.
%  %\hspace{2mm}\For{each minibatch b in $\mathcal{B}$}
%  \hspace{2mm}\For{each timestep $t$}
%  %\hspace{2mm}\For{each x $\in$ X \textbackslash $S_{i-1}$}
% %  \State $Rep_E^{b-1}$ = Pre-trained VGG-16 features($E_{b-1}$)
% %  \State $Rep_I^{b}$ = Pre-trained VGG-16 features($I_b$)
% \State Extract a minibatch of data from $\mathcal{B}$
% \State $u_i$ , $u_j$ = Features (maybe pre-trained) of image $i$ and $j$
% \State Let $D_{ij}^o$ be the pairwise distance between instance i from E and j from I and $D_{ij}^n$ be the pairwise distance between instance i and j from I
% %  \State $select_I$ = S($Rep_E^{b-1}, Rep_I^{b}$)
% %  \State S($Rep_E^{b-1}, Rep_I^{b}$) 
% \State S($D_{ij}^o, D_{ij}^n ; \theta$) is the selection network using representations of existing/representative set E and of incoming mini batch I.
% %  \tr{Write the formula for selection network.} 
% %  $D_{i,j} = u_i^T \theta u_j$ / $D_{ij} = 1 - \sigma(\theta^T [u_i, u_j]) $, $z_{ij} = argmin_z \sum_{i}\sum_{j} D_{i,j}^o z_{ij}^o + \sum_{ij} D_{i,j}^n z_{ij}^n$, $s_j = \frac{1}{\xi} max(\sum_i z_{ij}^n,\xi)$.
%  $D_{i,j} = ||(u_i - u_j)||_p$. Solve the convex optimisation problem $argmin_z \sum_{i}\sum_{j} D_{i,j}^o z_{ij}^o + \sum_{ij} D_{i,j}^n z_{ij}^n$ where $z^o$ and $z^n$ are the output variables.
%  \State Calculate: $s_j = \frac{1}{\xi} max(\sum_i z_{ij}^n,\xi)$ where $\xi$ is a threshold value. $s_j$ will be 0 for the unselected instances and 1 for the selected ones.
%   \State $E \longleftarrow E \bigcup \{j | s_j \geq \xi\}$
% %  \State  Select a subset of size $k$ , say $M_i$ such that they yield the maximum value in $fv$
% %   \State  TrLoss = LossN($select_I , w_{b-1})$ %\textit{NetF} is the forward propagation portion of \textit{Net}.
%  % \State $p_j(\theta) = s_j (\theta) / \sum_k s_k(\theta)$
%   \State  $TrLoss(\theta,\phi) = \sum_j s_j(\theta) Loss_j(\phi_{t-1})$ 
%   %* CE Loss($b_i, w_{b-1}$) where $b_i$ is an instance in mini batch b.
% %   \tr{write the actual training formula with selected examples}
%  \State Calculate: $\nabla_{\phi} Trloss(\theta,\phi_{t-1}) = \sum_{j\in training data} (s_j(\theta) \nabla_{\phi} Loss(x_j,y_j,\phi_{t-1}) $
%  %\State $\nabla_{\theta} Trloss = \sum_j \nabla_{\theta} \log(p_j(\theta)) Loss_j(\phi_{t-1}) $
%  \State Calculate: $\hat{\phi}_t(\theta,\phi_{t-1})$ = $\phi_{t-1} - \eta \nabla_{\phi} TrLoss(\theta,\phi_{t-1})$
% %\State $w_b$ = \textit{Net}($select_I , w_{b-1}$) //Train the network \textit{Net} with the subset.
% %  \State  TsLoss = LossN(Test data , $w_b)$
%  \State  $TsLoss(\theta,\phi_{t-1}) = \sum_{k\in test data} NewLoss(x_k, y_k , \hat{\phi}_{t}(\theta,\phi_{t-1}))$
%  \State $\theta_t$ = $\theta_{t-1} - \eta \nabla TsLoss(\theta_{t-1})$ //Update selection network parameters
%  \State $\phi_t$ = $\phi_{t-1} - \eta \nabla TrLoss(\theta,\phi_{t-1})$ //Update classification network parameters
%  %\State $Rep_E^b$ = Synth($w_b$, TrLoss, TsLoss)
%  %\State Synth($\dots$) is a synthesis network to produce representations from $E$ using model parameters.
% %  \State $Rep_E^b$ = LSH($Rep_E^{b-1}, Rep_I^b)$ // LSH($\dots$) finds the most similar instances in representative set which are closer to the incoming mini batch using method of indexing.
%  \EndFor
%  \State \textbf{Output:}
%  \State $w$ : Trained model parameters
%  \State $E$ : Final representative set
%  \end{algorithmic}
% \end{algorithm}


% \begin{algorithm}
%  \caption{: Coupled Subset Training}
%  \label{algo:submodular}
%  \begin{algorithmic}[1]
 
%  \State \textbf{Input:}
%  \State \hspace{2mm} Training data
%  \State \hspace{2mm} Test data
% %  \State \hspace{2mm} $k$: Subset cardinality
%  \State \textbf{Process:}\\
%   \hspace{2mm} Training set is partitioned into existing set E and incoming set I which is further partitioned into mini batches $\mathcal{B}$.
%  \hspace{2mm}\For{each minibatch b in $\mathcal{B}$}
 
% \State $u_i$ , $u_j$ = Pre-trained features of image $i$ and $j$

% \State S($D_{ij}^o, D_{ij}^n ; \theta$) is the selection network using representations of existing/representative set E and of incoming mini batch I.
%  $D_{i,j} = ||(u_i - u_j)||_p, z_{ij} = argmin_z \sum_{i}\sum_{j} D_{i,j}^o z_{ij}^o + \sum_{ij} D_{i,j}^n z_{ij}^n$, $s_j = \frac{1}{\xi} max(\sum_i z_{ij}^n,\xi)$.
%   \State $E \longleftarrow E \bigcup \{j | s_j \geq \xi\}$

%   \State  $TrLoss(\theta,\phi) = \sum_j s_j(\theta) Loss_j(\phi_{t-1})$ 
%  \State Calculate: $\nabla_{\phi} Trloss(\theta,\phi_{t-1}) = \sum_{j\in training data} (s_j(\theta) \nabla_{\phi} Loss(x_j,y_j,\phi_{t-1}) $
 
%  \State Calculate: $\hat{\phi}_t(\theta,\phi_{t-1})$ = $\phi_{t-1} - \eta \nabla_{\phi} TrLoss(\theta,\phi_{t-1})$

%  \State  $TsLoss(\theta,\phi_{t-1}) = \sum_{k\in test data} NewLoss(x_k, y_k , \hat{\phi}_{t}(\theta,\phi_{t-1}))$
%  \State $\theta_t$ = $\theta_{t-1} - \eta \nabla TsLoss(\theta_{t-1})$
 
%  \EndFor
%  \State \textbf{Output:}
%  \State $w$ : Trained model parameters
%  \State $E$ : Final representative set
%  \end{algorithmic}
% \end{algorithm}
